Effect of temperature anisotropy on the dynamics of geodesic acoustic modes

In this work, we revisit the linear gyro-kinetic theory of geodesic acoustic modes (GAMs) and derive a general dispersion relation for an arbitrary equilibrium distribution function of ions. A bi-Maxwellian distribution of ions is then used to study the effects of ion temperature anisotropy on GAM frequency and growth rate. We find that ion temperature anisotropy yields sensible modifications to both the GAM frequency and growth rate as both tend to increase with anisotropy and these results are strongly affected by the electron to ion temperature ratio.

==> Abstract.tex <==
\addcontentsline{toc}{chapter}{Abstract} \markboth{Abstract}{}
\begin{center}
\section*{Abstract}   
\end{center}

The MHD (\textbf{M}agneto\textbf{H}ydro\textbf{D}ynamics) model is used to study the macroscopic behavior of a plasma. The three types of waves that can be described by this model are the shear Alfven wave, the slow magneto-sonic waves and the fast magneto-sonic wave. Winsor et al \textcolor{blue}{\cite{winsor}} in 1968, showed that in toroidal systems with geodesic curvature, an electrostactic acoustic mode occurred with perpendicular motion of plasma with respect to the magnetic field.

 Our aim in this work is to the reproduce the result obtained by Winsor et al \textcolor{blue}{\cite{winsor}}, using an MHD model with a polytropic closure relation and to perform a similar analysis but now considering a double adiabatic closure relation.

==> title.tex <==
\begin{titlepage}
%\includegraphics[width=0.4\textwidth]{./fusion}~\\[1cm]
\begin{center}

%\HRule \\[0.4cm]

{\huge \bfseries Gyro-kinetic investigation of the dynamics of  geodesic acoustic modes\\[0.4cm] }

%\HRule \\[0.5cm]
J.N. SAMA$^1$, A. Biancalani$^{2,3}$, A. Bottino$^3$, I. Chavdarovski$^4$, D. Del Sarto$^1$, A. Ghizzo$^1$, T. Hayward-Schneider$^3$, B. Rettino$^3$ and F. Vannini$^3$\\
%{\large  Written by : }\\[0.5cm]
$^1$Institut Jean Lamour UMR 7198, Université de Lorraine- CNRS, Nancy, France\\
$^2$Léonard de Vinci Pôle Universitaire, Research Center, Paris La Défense, France\\
$^3$Max Planck Institute for Plasma Physics, Garching, Germany\\
$^4$Korea Institute of Fusion Energy, Daejeon, South Korea\\
%{\large J.N. SAMA^1, A. Biancalani^{2,3}, A. Bottino^3, I. Chavdarovski^4, D. Del Sarto^1, A. Ghizzo^1, T. Hayward-Schneider^3, M. Lesur^1, B. Rettino^3 and F. Vannini^3}\\[0.5cm]
%{\large  l'institut Jean Lamour UMR 7198}\\[0.5cm]
\vspace{10mm}
%\textsc{\Large }\\[0.5cm]
% Title
%\includegraphics[width=1\textwidth]{./bottom}~\\[1cm]
\vfill
% Bottom of the page
%{\large \today}
\end{center}
\end{titlepage}
